A computational proof of the linear Arithmetic Fundamental Lemma of GL$_4$

Let $K/F$ be an unramified quadratic extension of non-Archimedian local fields with residue character not equals to 2. We prove the linear Arithmetic Fundamental Lemma for GL$_4$ with the unit element in the spherical Hecke Algebra. In this article, all measures are normalized by its hyperspecial subgroup.

==> Compute/Acknowledgement.tex <==
The author would like to thank Professor Wei Zhang for his suggestion on topics for the author's Ph.D thesis. The author would like to thank Prof. Ben Howard for his interests and discussions of general orbital integrals in bi-quadratic case and invariant polynomials. 


==> Compute/Command/DoubleStructure.tex <==
% Test functions


% The resultant proof in double structures

\newcommand\hof{\Hom_F(U_x,V/U_x)}
\newcommand\dhopa{\Hom_{\baso'_1,\baso_1''}(U_x,V/U_x)}
\newcommand\dhoma{\Hom_{\baso'_1,\overline{\baso_1''}}(U_x,V/U_x)}
\newcommand\dhtpa{\Hom_{\baso'_2,\baso_2''}(U_x,V/U_x)}
\newcommand\dhtma{\Hom_{\baso'_2,\overline{\baso_2''}}(U_x,V/U_x)}
\newcommand\dhipa{\Hom_{\baso'_i,\baso''_i}(U_x,V/U_x)}
\newcommand\dhima{\Hom_{\baso'_i,\overline{\baso''_i}}(U_x,V/U_x)}

%The following are short notations

\newcommand\hopa{E_+^{\baso_1}}
\newcommand\homa{E_-^{\baso_1}}
\newcommand\htpa{E_+^{\baso_2}}
\newcommand\htma{{E_-^{\baso_2}}}
\newcommand\hipa{E_+^{\baso_i}}
\newcommand\hipe{E_\pm^{\baso_i}}
\newcommand\hima{{E_-^{\baso_i}}}
\newcommand\hime{{E_\mp^{\baso_i}}}
%Intersection Numeber Symbol

\newcommand\intnu{\mathrm{Int}(\ACj)}

% The K-normalizer 

\newcommand\ek[1]{\ep_{K,#1}}
\newcommand\ef[1]{\ep_{F,#1}}

%Oh my god
\newcommand{\farc}[2]{\frac{#2}{#1}}

\newcommand\ft{f(P_t)}

% Invariant Polynomial

\newcommand\iv[1]{P_{#1}}
\newcommand\ivv[1]{P^{> r}_{#1}}
\newcommand\ivvv[1]{P^{\leq r}_{#1}}


% Division Algebras

\newcommand{\D}{D}
\newcommand{\DD}{D^\times}
\newcommand{\DDD}{\OO D}
\newcommand{\DDDD}{\OO D^\times}

% G- The F-side 

\def\g{\mathrm{Mat}_{2h}(F)}
\def\gg{\mathbf{G}_{2h}(F)}
\def\ggg{\mathrm{Mat}_{2h}(\OO F)}
\def\gggg{\mathbf{G}_{2h}(\OO F)}
\def\ggggg{\mathbf{G}_{2h}(\OO F/\pi)}

%Lie Algebra
\newcommand\lgggg{\mathfrak{g}_{2h}(\OO F)}
\newcommand\lgg{\mathfrak{g}_{2h}(F)}


% Haar-Measure F-side

\newcommand{\df}{\dd g}

% G- h could vary
\newcommand\gh[1]{\mathrm{Mat}_{2{#1}}(F)}
\newcommand\ggh[1]{\mathbf{G}_{2{#1}}(F)}
\newcommand\gggh[1]{\mathrm{Mat}_{2{#1}}(\OO F)}
\newcommand\ggggh[1]{\mathbf{G}_{2{#1}}(\OO F)}
\newcommand\gggggh[1]{\mathbf{G}_{2{#1}}(\OO F/\pi)}
% G- The FxF side

\def\ga{\mathrm{Mat}_{h}(F)\times \mathrm{Mat}_{h}(F)}
\def\gga{\mathbf{G}_{h}(F)\times \mathbf{G}_{h}(F)}
\def\ggga{\mathrm{Mat}_{2h}(\OO F)\times \mathrm{Mat}_{2h}(\OO F)}
\def\gggga{\mathbf{G}_{2h}(\OO F)\times \mathbf{G}_{2h}(\OO F)}
\def\ggggga{\mathbf{G}_{2h}(\OO F/\pi)\times \mathbf{G}_{2h}(\OO F/\pi)}

% K side before
%\newcommand{\E}[1]{\mathrm{C}(#1)}
%\newcommand{\EE}[1]{\mathrm{C}^\times(#1)}
%\newcommand{\EEE}[1]{\OO{ \mathrm{C}}(#1)}
%\newcommand{\EEEE}[1]{\OO{ \mathrm{C}^\times}(#1)}
%\newcommand{\Eo}[1]{\mathrm{C}(#1_1)}
%\newcommand{\EEo}[1]{\mathrm{C}^\times(#1_1)}
%\newcommand{\EEEo}[1]{\OO{ \mathrm{C}}(#1_1)}
%\newcommand{\EEEEo}[1]{\OO{ \mathrm{C}^\times}(#1_1)}
%\newcommand{\Et}[1]{\mathrm{C}(#1_2)}
%\newcommand{\EEt}[1]{\mathrm{C}^\times(#1_2)}
%\newcommand{\EEEt}[1]{\OO{ \mathrm{C}}(#1_2)}
%\newcommand{\EEEEt}[1]{\OO{ \mathrm{C}}^\times(#1_2)}
%\newcommand{\Ei}[1]{\mathrm{C}(#1_i)}
%\newcommand{\EEi}[1]{\mathrm{C}^\times(#1_i)}
%\newcommand{\EEEi}[1]{\OO{ \mathrm{C}}(#1_i)}
%\newcommand{\EEEEi}[1]{\OO{ \mathrm{C}}^\times(#1_i)}

%General Division Algebra K-side
\newcommand{\dE}{\mathrm{D_K}}
\newcommand{\dEE}{\mathbf{D_K}^\times}
\newcommand{\dEEE}{{\OO{D_K}}}
\newcommand{\dEEEE}{{\OO{D_K}}^\times}
\newcommand{\dEEEEE}{({\OO{D_K}}/\pi)^\times}
\newcommand{\dEo}{\mathrm{D_{K_1}}}
\newcommand{\dEEo}{\mathrm{D_{K_1}}^\times}
\newcommand{\dEEEo}{{\OO{D_{K_1}}}}
\newcommand{\dEEEEo}{{\OO{ D_{K_1}}}^\times}
\newcommand{\dEt}{\mathrm{D}_{K_2}}
\newcommand{\dEEt}{\mathrm{D}_{K_2}^\times}
\newcommand{\dEEEt}{{\OO D}_{K_2}}
\newcommand{\dEEEEt}{{\OO D}_{K_2}^\times}
\newcommand{\dEi}{\mathrm{D}_{K_i}}
\newcommand{\dEEi}{\mathrm{D}_{K_i}^\times}
\newcommand{\dEEEi}{{\OO {D_{K_i}}}}
\newcommand{\dEEEEi}{{\OO{D_{K_i}}^\times}}

%G- K side
\newcommand{\E}{\mathrm{Mat}_h(K)}
\newcommand{\Eh}[1]{\mathrm{Mat}_{#1}(K)}
\newcommand{\EE}{\mathbf{G}_h(K)}
\newcommand{\DEE}{\mathbf{G}^\Delta_h(K)}
\newcommand{\EEh}[1]{\mathbf{G}_{#1}(K)}
\newcommand{\EEE}{\mathrm{Mat}_h(\OO K)}
\newcommand{\EEEh}[1]{\mathrm{Mat}_{#1}(\OO K)}
\newcommand{\EEEE}{\mathbf{G}_h(\OO K)}
\newcommand{\DEEEE}{\mathbf{G}^\Delta_h(\OO K)}
\newcommand{\EEEEh}[1]{\mathbf{G}_{#1}(\OO K)}
\newcommand{\DEEEEh}[1]{\mathbf{G}^{\Delta}_{#1}(\OO K)}
\newcommand{\TEEEEh}[1]{\mathbf{G}^{t}_{#1}(\OO K)}
\newcommand{\EEEEEh}[1]{\mathbf{G}_{#1}(\OO K/\pi)}
\newcommand{\Eo}{\mathrm{Mat}_h(K_1)}
\newcommand{\EEo}{\mathbf{G}_h(K_1)}
\newcommand{\EEEo}{\mathrm{Mat}_h(\OO{K_1})}
\newcommand{\EEEEo}{\mathbf{G}_h(\OO{K_1})}
\newcommand{\Et}{\mathrm{Mat}_h(K_2)}
\newcommand{\EEt}{\mathbf{G}_h(K_2)}
\newcommand{\EEEt}{\mathrm{Mat}_h(\OO{K_2})}
\newcommand{\EEEEt}{\mathbf{G}_h(\OO{K_2})}
\newcommand{\Ei}{\mathrm{Mat}_h(K_i)}
\newcommand{\EEi}{\mathbf{G}_h(K_i)}
\newcommand{\EEEi}{\mathrm{Mat}_h(\OO{K_i})}
\newcommand{\EEEEi}{\mathbf{G}_h(\OO{K_i})}

% G - FxF side

\newcommand{\W}{\mathrm{Mat}_h(F)\times \mathrm{Mat}_h(F)}
\newcommand{\WW}{\mathbf{G}_h(F)\times \mathbf{G}_h(F)}
\newcommand{\WWW}{\mathrm{Mat}_h(\OO F)\times \mathrm{Mat}_h(\OO F)}
\newcommand{\WWWW}{\mathbf{G}_h(\OO F)\times \mathbf{G}_h(\OO F)}
\newcommand{\WWWWW}{\mathbf{G}_h(\OO F/\pi)\times \mathbf{G}_h(\OO F/\pi)}
\newcommand{\Wo}{\mathrm{Mat}_h(F_1)\times \mathrm{Mat}_h(F_1)}
\newcommand{\WWo}{\mathrm{C}(\blin_1)}
\newcommand{\WWWo}{\mathrm{Mat}_h(\OO{F_1})\times \mathrm{Mat}_h(\OO{F_1})}
\newcommand{\WWWWo}{\mathbf{G}_h(\OO{F_1})\times \mathbf{G}_h(\OO{F_1})}
\newcommand{\Wt}{\mathrm{Mat}_h(F_2)\times \mathrm{Mat}_h(F_2)}
\newcommand{\WWt}{\mathrm{C}(\blin_2)}
\newcommand{\WWWt}{\mathrm{Mat}_h(\OO{F_2})\times \mathrm{Mat}_h(\OO{F_2})}
\newcommand{\WWWWt}{\mathbf{G}_h(\OO{F_2})\times \mathbf{G}_h(\OO{F_2})}
\newcommand{\Wi}{\mathrm{Mat}_h(F_i)\times \mathrm{Mat}_h(F_i)}
\newcommand{\WWi}{\mathrm{C}(\blin_i)}
\newcommand{\WWWi}{\mathrm{Mat}_h(\OO{F_i})\times \mathrm{Mat}_h(\OO{F_i})}
\newcommand{\WWWWi}{\mathbf{G}_h(\OO{F_i})\times \mathbf{G}_h(\OO{F_i})}


%Lie Algebra, used in unipotent part
\newcommand\LEE{\mathfrak{g}_{a}({K})}
\newcommand\LEEEE{\mathfrak{g}_{a}(\OO{K})}
\newcommand\LDEEEE{\mathfrak{g}^\Delta_{a}}
\newcommand\LTEEEE{\mathfrak{g}^t_{a}(\OO{K})}
% Lie Algebra

\newcommand\LEEo{\mathfrak{g}_{h}({K_1})}
\newcommand\LEEEEo{\mathfrak{g}_{h}(\OO{K_1})}
\newcommand\LEEEEt{\mathfrak{g}_{h}(\OO{K_2})}
\newcommand\LEEEEi{\mathfrak{g}_{h}(\OO{K_i})}
\newcommand\LEEt{\mathfrak{g}_{h}({K_2})}
\newcommand\LEEi{\mathfrak{g}_{h}({K_i})}

% Haar -measure K-side

\newcommand{\dko}{\dd k_1}
\newcommand{\dkt}{\dd k_2}
% Homogeneous spaces


\def\SS{\mathfrak{S}_h(F)}
\newcommand\SSh[1]{\mathfrak{S}_{#1}(F)}
\def\SSS{\mathfrak{S}_h(\OO F)}
\newcommand\SSSh[1]{\mathfrak{S}_{#1}(\OO F)}
\newcommand\sssh[1]{\mathcal{H}_{#1}(\OO F)}
\newcommand\SSShr[2]{\mathfrak{S}_{#1}^{>{#2}}(\OO F)}
\newcommand\SSShrr[2]{\mathfrak{S}_{#1}^{\leq{#2}}(\OO F)}


\def\OSS{\mathfrak{S}^\circ_h(F)}
\newcommand\OSSh[1]{\mathfrak{S}^\circ_{#1}(F)}
\def\OSSS{\mathfrak{S}^\circ_h(\OO F)}
\newcommand\OSSSh[1]{\mathfrak{S}^\circ_{#1}(\OO F)}
\newcommand\OSSShr[2]{\mathfrak{S}^\circ_{#1}^{>{#2}}(\OO F)}
\newcommand\OSSShrr[2]{\mathfrak{S}^\circ_{#1}^{\leq{#2}}(\OO F)}


% PSC coordinate

\newcommand\sss{\mathcal H_h(F)}
\newcommand\sso{\mathcal H_h^\circ(F)}
\newcommand\ssa{\mathcal H_a(F)}
\newcommand\ssss[2]{\mathcal H^{>#1}_{#2}(\OO F)}
\newcommand\sssss{\mathcal H(\OO F)}
\newcommand\ssssss[3]{\mathcal H^{>#1}_{#2,#3}(\OO F)}
\newcommand\sssssssss[2]{\mathcal H^{=0}_{#1,#2}(\OO F)}
% Eigenvalue cutting condition
\newcommand\SSSS[3]{\mathfrak{S}^{>#1}_{#2,#3}(F)}
\newcommand\SSSSSSSS[3]{\mathfrak{S}^{\leq#1}_{#2,#3}(F)}
\newcommand\SSSSSSS[3]{\mathfrak{S}^{\leq#1}_{#2,#3}(\OO F)}
\newcommand\SSSSSS[3]{\mathfrak{S}^{>#1}_{#2,#3}(\OO F)}
\newcommand\SSSSS[3]{\mathfrak{S}^{\leq#1}_{#2,#3}(F)}

% Parabolic subgroups P-F side

\newcommand{\pF}{\mathbf{P}_{F,U}(F)}
\newcommand{\PF}{\mathbf{P}_{F,U}(\OO F)}
\newcommand{\PU}{\mathbf{P}_{F,U}(\OO F)}
\newcommand{\PFF}{\mathbf{P}_{F,U}(\OO F/\pi)}
\newcommand{\PFFF}[1]{\mathbf{P}_{F,#1}(\OO F)}

% Lie Algebra

\newcommand{\LPF}{\mathfrak{p}_{F}(\OO F)}

% Haar-Measure

\newcommand{\dpf}{\dd p_F}
\newcommand{\dpp}{\dd p}


\newcommand{\pK}{\mathbf{P}_{K,U}(K_1)}
\newcommand{\PK}{\mathbf{P}_{K,U}(\OO {K_1})}
\newcommand{\PPK}{\mathbf{P}_{K,U}(\OO {K})}
\newcommand{\PKt}{\mathbf{P}_{K,U}(\OO {K_2})}
\newcommand{\PKi}{\mathbf{P}_{K,U}(\OO {K_i})}
\newcommand{\PKK}{\mathbf{P}_{K,U}(\OO {K_1}/\pi)}
\newcommand{\PKKK}[1]{\mathbf{P}_{K,#1}(\OO {K_1})}

% Lie Agelra
\newcommand{\LPK}{\mathfrak{p}_{K}(\OO{K_1})}
\newcommand{\LPKK}{\mathfrak{p}_{U,K}(\OO{K})}
\newcommand{\lpK}{\mathfrak{p}_{K}({K_1})}
\newcommand{\LPKt}{\mathfrak{p}_{K}(\OO{K_2})}
\newcommand{\LPKi}{\mathfrak{p}_{K}(\OO{K_i})}
\newcommand{\lpKt}{\mathfrak{p}_{K}({K_2})}
\newcommand{\lpKi}{\mathfrak{p}_{K}({K_i})}

% Haar - Measure

\newcommand{\dpo}{\dd p_1}
\newcommand{\dpt}{\dd p_2}
\newcommand{\dpi}{\dd p_i}


% Homogeneous space P-side

\newcommand{\TT}{\mathfrak{P}_{U}(\OO F)}
% Eigenvalue cutting condition
\def\TTT{\mathfrak{P}_{U}^{>r}(\OO F)}
\newcommand\OTTT{\one_{\TTT}}
\newcommand\TTTT[1]{\mathfrak{P}_{U_{#1}}^{>r}(\OO F)}


% Eigenvalue cutting condition
\newcommand{\tT}{\mathcal{P}_{U}(\OO F)}
\def\ttt{\mathcal{P}_{U}^{>0}(\OO F)}
\newcommand\Ottt{\one_{\ttt}}
\newcommand\tttt[1]{\mathcal{P}_{U_{#1}}^{>r}(\OO F)}


% Grassmanion K-side
\def\Gr{\mathrm{Gr}_{h,a}(K)}
\def\GR{\mathrm{Gr}_{h,a}(\OO K)}

% Flag Variety

\newcommand\Fl{\mathrm{Fl}_a(K)}
\newcommand\FL{\mathrm{Fl}_a(\OO K)}

%Unipotnet U-F side

\newcommand{\uF}{\mathbf{U}_{2m,2n}(F)}
\newcommand{\UF}{\mathbf{U}_{2m,2n}(\OO F)}
\newcommand{\uK}{\mathbf{U}_{2m,2n}(K)}
\newcommand{\UK}{\mathbf{U}_{2m,2n}(\OO K)}
\newcommand{\UKo}{\mathbf{U}_{2m,2n}(\OO{K_1})}
\newcommand{\UKt}{\mathbf{U}_{2m,2n}(\OO{K_2})}

%Lie Algebras

\newcommand{\LUF}{\mathfrak{u}_{F}(\OO{F})}
\newcommand{\LUKo}{\mathfrak{u}_{K}(\OO{K_1})}
\newcommand{\LUKt}{\mathfrak{u}_{K}(\OO{K_2})}
\newcommand{\LUKi}{\mathfrak{u}_{K}(\OO{K_i})}

\newcommand{\luf}{\mathfrak{u}_{F}(F)}
\newcommand{\luko}{\mathfrak{u}_{K}(K_1)}
\newcommand{\lukt}{\mathfrak{u}_{K}(K_2)}
\newcommand{\luki}{\mathfrak{u}_{K}(K_i)}

% Homogeneous space U-side


\newcommand{\UU}{\mathfrak{U}_{m,n}(\baso',\baso'')}
\newcommand{\uuu}{\mathcal{U}_{U}(\OO F)}


% Levi M-F side

\newcommand{\mF}{\mathbf{M}_{2m,2n}(F)}
\newcommand{\MF}{\mathbf{M}_{2m,2n}(\OO F)}
\newcommand{\mK}{\mathbf{M}_{2m,2n}(K)}
\newcommand{\MK}{\mathbf{M}_{2m,2n}(\OO K)}


% Homogeneous space

\newcommand{\MMM}{\SSSh m\times \SSSh n}
\newcommand{\MM}{\SSh m\times \SSh n}



% Eigenvalue condition

\newcommand{\eico}{\vv_F\left(1-\frac1\lambda\right)>r}
% Parabolic homogeneous subspaces




\newcommand{\baso}{\alpha}
\newcommand{\err}[1]{e_{#1_1,#1_2}}
\newcommand{\irr}[1]{i_{#1_1,#1_2}}
\newcommand{\ert}{\err{\tau}}
\newcommand{\irt}{\irr{\tau}}
\newcommand{\ero}{\err{\biso}}
\newcommand{\iro}{\irr{\biso}}

\newcommand{\ds}[1]{(#1_1,#1_2)}
\newcommand{\dds}[1]{\langle #1_1,#1_2\rangle}
\newcommand{\za}[1]{#1_1(\zeta)}
\newcommand{\zi}[1]{#1_2(\zeta)}
\newcommand{\zo}[1]{#1_i(\zeta)}
\newcommand{\zop}[1]{#1_i'(\zeta)}
\newcommand{\zopp}[1]{#1_i''(\zeta)}
%\newcommand{\zaba}{\za\baso}
\newcommand\zaba{x_0}
\newcommand{\zabap}{\zap\baso}
\newcommand{\zabapp}{\zapp\baso}
\newcommand{\zap}[1]{#1_1'(\zeta)}
\newcommand{\zapp}[1]{#1_1''(\zeta)}
\newcommand{\zip}[1]{#1_2'(\zeta)}
\newcommand{\zipp}[1]{#1_2''(\zeta)}
\newcommand{\zabi}{\za\blin}
\newcommand{\zabia}{\za{\blin^\sigma}}
\newcommand{\zobi}{\zo\blin}
\newcommand{\zobia}{\zo{\blin^\sigma}}
\newcommand{\zobap}{\zop\baso}
\newcommand{\zobapp}{\zopp\baso}
\newcommand{\zabaa}{\za\baso^{-1}}
\newcommand{\ziba}{\zi\baso}
\newcommand{\zibap}{\zip\baso}
\newcommand{\zibapp}{\zipp\baso}
\newcommand{\zibi}{\zi\blin}
\newcommand{\zibia}{\zi{\blin^\sigma}}
\newcommand{\zibaa}{\zi\baso^{-1}}

\newcommand\zaca{\za{\baso^\sigma}}
\newcommand\zica{\zi{\baso^\sigma}}

\newcommand{\ctro}[1]{\mathrm{C}(#1_1)}
\newcommand{\ctrt}[1]{\mathrm{C}(#1_2)}
\newcommand{\ctri}[1]{\mathrm{C}(#1_i)}

%Terminologies

\newcommand{\dbs}{double structure }
\newcommand{\psc}{polar stereographic coordinate }
\newcommand{\ipo}{invariant polynomial }


==> Compute/Response.tex <==
\section{Changes Made}

This paper has been rewritten. The previous paper can be found at: https://arxiv.org/pdf/1907.00090.pdf. It has the following concerns.
\[itemize]{
\item Introduction is Dry.
\item Lots of Grammar mistakes.
\item Too technical. A lot of formulas do not have a clear picture. 
\item Not enough landmark or section map to let the reader know where we are. Especially the later sections. 
}

Besides, the author also founds the following disadvantage of the old version
\[itemize]{
\item Heavily use of $\phi_h$ without a clear picture of this function. 
	}

In this version those concerns are all clear. 

\[itemize]{
\item I made the introduction to the best as I can.
\item I made the purpose of each section clear at the beginning of each section. I also pointed out which part can be skip by reader if they want to read the paper fast.
\item I have introduced double structures, which are naturally parameters in the orbital integrals of the linear AFL conjecture.
\item In fact all computation is happening on a homogeneous space $\SS$. the function $\phi_h$ in the old paper is a characteristic function on its integral points $\SSS$.
\item With the section introducing double structures, the definition of invariant polynomial seems more natural.
\item I explained in a single section the method of my integration is the integration by fibration. This method can also be used in other scenarios. With this section, the reader can have a clearer picture why I am doing fib rations in the paper.
\item The author checked carefully with grammars and words in the paper.(Although it might still be some left)
	}
The only concern for the new version is that it gets longer. I attached another letter to explain the issue and trade-offs. 

\newpage



==> Compute/SecondReferee.tex <==
\newpage
\section{Note to referees}
Dear Referee:

\vspace{0.5cm}
Thank you very much for all those helpful suggestions, here is a second revision version. 
\[itemize]{
\item Fixes all typos and I let it reviewed by a native speaker.
\item This paper has been updated so all proof works for characteristic 2.
\item I have updated Section \S\ref{md}. I have introduced more intuitive structures, the angle bisectors in Definition \ref{ie} is helpful to understand most of the proofs.
\item I have updated the proof of the key Theorem \ref{wodemaya} with the operator $\Theta_\pm$, I believe this proof make more sense.
\item Some other changes that could be simplified by using the inner and outer angle bisectors introduced in Definition \ref{ie}. Besides the Section \ref{md}, it appears in Lemma \ref{inva}, Lemma \ref{kuaidian}, Lemma\ref{nimeimei}, Section \S\ref{popo} and Section \S\ref{lati}. You may find it simplified things and it is helpful.
	}

Here are some concerns of the referee and I am happy to answer all of them as follows.
\[ex]{The domain of integration in \eqref{xiaotina} should be $C(\tau_1)\times C(\tau_2)$?
	}
\[proof]{No, it has to be $C(\tau_1)\times C(\tau_1)$, it is not a typo. I confirm here $u_2\in C(\tau_1)$. It doesn't break the symmetry of $\tau_1$ and $\tau_2$ because $g$ has the information relating $\tau_1$ and $\tau_2$. To change the role, we could replace $\tau_1$ by $\tau_2$ and replace $g$ by $g^{-1}$.}

\[ex]{The problem regarding $\ACj$?}
\[proof]{That's a good point. Now in the paper the symbol $\ACj$ refers to a double structure on division algebra as I said in the paper $\ACj=(\varphi_1,\varphi_2)$. I know originally by $\ACj$ I want to represent an element in division algebra, but I no longer need to do so.}

\[ex]{Divide two volume forms}
\[proof]{I have add sentences before Theorem \ref{fansile} to help reader understand this. I am thinking when we have an exact sequence of vector spaces
$$
\xymatrix{0\ar[r]& U\ar[r]&V\ar[r]&W\ar[r]&0}.
$$
If $\bigwedge$ means the highest wedge product of a vector space. Then we have naturally a one-dimensional space isomorphism 
$$\bigwedge V = \bigwedge U\otimes \bigwedge W,$$
then the division of two non-zero vectors has a clear meaning. A vector in $\bigwedge V$ divide by a vector in $\bigwedge W$ is a vector in $\bigwedge U$ by solving the equation $v=w\otimes x$ for $x$ where $v\in \bigwedge V$ and $w\in \bigwedge W$. The solution here is unique.

So when dividing volume forms, we are actually dividing the highest form of cotangent vectors at every point of the manifold. The result would only located in the highest form of cotangent spaces of the submanifold at every point.
	}

Thank you very much for all of those helpful suggestions. Please also stay safe and healthy.



==> Compute/etc.tex <==
Title: A proof of the linear Arithmetic Fundamental Lemma for $\GL_4$


==> PlainPaper/Command/control.tex <==



==> PlainPaper/Command/history/linear.tex <==
%ini/Command
\newcommand{\basis}[2]{\rrrr{#1_1}{#1_2}{\cdots}{#1_#2}}
\newcommand{\coro}[2]{\cccc{#1_1}{#1_2}{\vdots}{#1_#2}}
\newcommand{\coros}[4]{\cccc{#1_1#2#3_1}{#1_2#2#3_2}{\vdots}{#1_#4#2#3_#4}}
\newcommand{\corov}[3]{\cccc{#1_1#2}{#1_2#2}{\vdots}{#1_#3#2}}
%The following are only for examples
\newcommand{\rrce}[6]{\left(\begin{array} {ccc}\hline
\multicolumn{1}{|c}{#1} & #2	&\multicolumn{1}{c|}{#3}	\\\hline
#4 & #5	&#6	\\
\end{array}
\right)}

\newcommand{\ccre}[6]{\left(\begin{array} {c|c|}\cline{2-2}
#1 & #2	\\
#3 & #4	\\
#5 & #6	\\\cline{2-2}
\end{array}
\right)}

\newcommand{\mme}[4]{\left(\begin{array} {cc}\cline{2-2}
#1 & \multicolumn{1}{|c|}{#2}\\\cline{2-2}
#3 & #4\\
\end{array}
\right)}
%The following are for determinants

\newcommand{\dets}[4]{\left|\begin{array} {ccccc}
#1_{11}	&#1_{12}&#1_{13}&\cdots	& #1_{1#4}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#2 1}	&#1_{#2 2}&#1_{#2 3}&\cdots	& #1_{#2 #4}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#3 1}	&#1_{#3 2}&#1_{#3 3}&\cdots	& #1_{#3 #4}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#4 1}	&#1_{#4 2}&#1_{#4 3}&\cdots	& #1_{#4 #4}\\
\end{array}
\right|}

\newcommand{\detu}[3]{\left|\begin{array} {ccccc}
#1_{11}	&#1_{12}&#1_{13}&\cdots	& #1_{1#3}\\
        &#1_{2 2}&#1_{2 3}&\cdots	& #1_{2 #3}\\
        &       &#1_{#2 3}&\cdots	& #1_{#2 #3}\\
    	&      &    	&\cdots	&\cdots	\\
	&&&   & #1_{#3 #3}\\
\end{array}
\right|}

\newcommand{\detdia}[4]{\left|\begin{array} {ccccc}
#1	&    &      &       &       \\
        &#2&      &   	&       \\
        &       &#3& 	&       \\
    	&      &    	&\ddots	&	\\
	&&&   & #4\\
\end{array}
\right|}

\newcommand{\deta}[5]{\left|\begin{array} {ccccc}
#1_{11}	&#1_{12}&#1_{13}&\cdots	& #1_{1#5}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#3 1}+#2 #1_{#4 1}	&#1_{#3 2}+#2 #1_{#4 2}&#1_{#3 3}+#2 #1_{#4 3}&\cdots	& #1_{#3 #5}+#2 #1_{#4 #5}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#4 1}	&#1_{#4 2}&#1_{#4 3}&\cdots	& #1_{#4 #5}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#5 1}	&#1_{#5 2}&#1_{#5 3}&\cdots	& #1_{#5 #5}\\
\end{array}
\right|}

%\newcommand{\detaa}[5]{\left|\begin{array} {ccccc}
%#1_{11}	&#1_{12}&#1_{13}&\cdots	& #1_{1#5}\\
%\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
%#1_{#3 1}+#2_{#4 1}	&#1_{#3 2}+#2_{#4 2}&#1_{#3 3}+#2_{#4 3}&\cdots	& #1_{#3 %#5}+#2_{#4 #5}\\
%\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
%#1_{#4 1}	&#1_{#4 2}&#1_{#4 3}&\cdots	& #1_{#4 #5}\\
%\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
%#1_{#5 1}	&#1_{#5 2}&#1_{#5 3}&\cdots	& #1_{#5 #5}\\
%\end{array}
%\right|}

\newcommand{\dett}[1]{\left|\begin{array}{c}#1\end{array}\right|}

\newcommand{\detaao}[4]{\left|\begin{array} {cccc}
#1_{11}	&#1_{12}&\cdots	& #1_{1#4}\\
\cdots	&\cdots	&\cdots	&\cdots\\
#2_{#3 1}	&#2_{#3 1}&\cdots	& #2_{#3 1}\\
\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#4 1}	&#1_{#4 2}&\cdots	& #1_{#4 #4}\\
\end{array}
\right|}

\newcommand{\detaa}[4]{\left|\begin{array} {cccc}
#1_{11}	&#1_{12}&\cdots	& #1_{1#4}\\
\cdots	&\cdots	&\cdots	&\cdots\\
#2_{#3 1}+#1_{#3 1}	&#2_{#3 1}+#1_{#3 2}&\cdots	& #2_{#3 1}+#1_{#3 #4}\\
\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#4 1}	&#1_{#4 2}&\cdots	& #1_{#4 #4}\\
\end{array}
\right|}

\newcommand{\detm}[4]{\left|\begin{array} {cccc}
#1_{11}	&#1_{12}&\cdots	& #1_{1#4}\\
\cdots	&\cdots	&\cdots	&\cdots\\
#2#1_{#3 1}	&#2#1_{#3 2}&\cdots	& #2#1_{#3 #4}\\
\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#4 1}	&#1_{#4 2}&\cdots	& #1_{#4 #4}\\
\end{array}
\right|}
%The following are for elementary matrices

\newcommand{\elm}[2]{\bordermatrix{%
& 	&	&i	&	&	\cr
&#1 	&	&	&	&	\cr
&	&\ddots	&	&	&	\cr
i&	&	&#2	&	&	\cr
&	&	&	&\ddots	&	\cr
&	&	&	&	&#1	\cr
}}
\newcommand{\els}[1]{\bordermatrix{
& 	&	&	&	&	&	&	\cr
&#1 	&	&	&	&	&	&	\cr
&	&\ddots	&	&	&	&	&	\cr
i&	&	&0	&	&#1	&	&	\cr
&	&	&	&\ddots	&	&	&	\cr
j&	&	&#1	&	&0	&	&	\cr
&	&	&	&	&	&\ddots	&	\cr
&	&	&	&	&	&	&#1	\cr
}}

\newcommand{\ela}[2]{\bordermatrix{
& 	&	&	&	&j	&	&	\cr
&#1 	&	&	&	&	&	&	\cr
&	&\ddots	&	&	&	&	&	\cr
i&	&	&#1	&	&#2	&	&	\cr
&	&	&	&\ddots	&	&	&	\cr
&	&	&	&	&#1	&	&	\cr
&	&	&	&	&	&\ddots	&	\cr
&	&	&	&	&	&	&#1	\cr
}}

%The following are some some particular Matrices.
\newcommand{\mat}[5]{(#1_{#2#3})_{\substack{1\leq #2 \leq #4 \\ 1\leq #3 \leq #5}}}
\newcommand{\mato}[5]{(#1)_{\substack{1\leq #2 \leq #4 \\ 1\leq #3 \leq #5}}}

\newcommand{\mm}[4]{\begin{pmatrix}
#1 & #2\\
#3 & #4\\
\end{pmatrix}}

\newcommand{\nmm}[4]{\begin{array} {cc}
#1 & #2\\
#3 & #4\\
\end{array}
}

\newcommand{\hmm}[4]{\left(\begin{array} {c;{2pt/2pt}c}
#1 & #2\\ \hdashline[2pt/2pt]
#3 & #4\\
\end{array}
\right)}

\newcommand{\nhmm}[4]{\begin{array} {c;{2pt/2pt}c}
#1 & #2\\ \hdashline[2pt/2pt]
#3 & #4\\
\end{array}
}

\newcommand{\rrc}[6]{\left(\begin{array} {ccc}
#1 & #2	&#3	\\
#4 & #5	&#6	\\
\end{array}
\right)}

\newcommand{\nrrc}[6]{\begin{array} {ccc}
#1 & #2	&#3	\\
#4 & #5	&#6	\\
\end{array}
}


\newcommand{\ccr}[6]{\left(\begin{array} {cc}
#1 & #2	\\
#3 & #4	\\
#5 & #6	\\
\end{array}
\right)}

\newcommand{\nccr}[6]{\begin{array} {cc}
#1 & #2	\\
#3 & #4	\\
#5 & #6	\\
\end{array}
}


\newcommand{\mmm}[9]{\left(\begin{array} {ccc}
#1 & #2 & #3\\
#4 & #5 & #6\\
#7 & #8 & #9\\
\end{array}
\right)}

\newcommand{\hmmm}[9]{\left(\begin{array} {c;{2pt/2pt}c;{2pt/2pt}c}
#1 & #2 & #3\\ \hdashline[2pt/2pt]
#4 & #5 & #6\\ \hdashline[2pt/2pt]
#7 & #8 & #9\\
\end{array}
\right)}

\newcommand{\nmmm}[9]{\begin{array} {ccc}
#1 & #2 & #3\\
#4 & #5 & #6\\
#7 & #8 & #9\\
\end{array}
}

\newcommand{\mms}[3]{\left(\begin{array} {cccc}
#1_{11}	&#1_{12}&\cdots	& #1_{1#3}\\
#1_{21}	&#1_{22}&\cdots	& #1_{2#3}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#1_{#2 1}	&#1_{#2 2}&\cdots	&#1_{#2#3}\\
\end{array}
\right)}


\newcommand{\mmhrs}[3]{\hrrrr{\ncccc{#1_{11}}{#1_{21}}{\vdots}{#1_{#2 1}}}{\ncccc{#1_{12}}{#1_{22}}{\vdots}{#1_{#1 2}}}{\ncccc{\cdots}{\cdots}{\ddots}{\cdots}}{\ncccc{#1_{1#3}}{b_{2#3}}{\vdots}{b_{#2#3}}}}

\newcommand{\mmhcs}[3]{\hcccc{\nrrrr{#1_{11}}{#1_{12}}{\cdots}{#1_{1#2 }}}{\nrrrr{#1_{21}}{#1_{22}}{\cdots}{#1_{2#1}}}{\nrrrr{\vdots}{\vdots}{\ddots}{\vdots}}{\nrrrr{#1_{#3 1}}{b_{#3 #2}}{\cdots}{b_{#2#3}}}}


\newcommand{\mmtrs}[3]{\left(\begin{array} {cccc}
#1_{11}	&#1_{21}&\cdots	& #1_{#3 1}\\
#1_{12}	&#1_{22}&\cdots	& #1_{#3 2}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#1_{1#2}	&#1_{2#2}&\cdots	&#1_{#3#2}\\
\end{array}
\right)}

\newcommand{\mmmm}[3]{\left(\begin{array} {cccc}
#111	&#121 &\cdots	& #1#31\\
#112	&#122 &\cdots	& #1#32\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#11#2	&#12#2&\cdots	&#1#3#2\\
\end{array}
\right)}

\newcommand{\upper}[2]{\left(\begin{array} {cccc}
#1_{11}	&#1_{12}&\cdots	& #1_{1#2}\\
	&#1_{22}&\cdots	& #1_{2#2}\\
	&	&\ddots	&\vdots	\\
	&	&	&#1_{#2#2}\\
\end{array}
\right)}

\newcommand{\upperm}[3]{\left(\begin{array} {cccc}
#3#1_{11}	&#1_{12}&\cdots	& #1_{1#2}\\
	&#3#1_{22}&\cdots	& #1_{2#2}\\
	&	&\ddots	&\vdots	\\
	&	&	&#3#1_{#2#2}\\
\end{array}
\right)}

\newcommand{\nupperm}[3]{\begin{array} {cccc}
#3#1_{11}	&#1_{12}&\cdots	& #1_{1#2}\\
	&#3#1_{22}&\cdots	& #1_{2#2}\\
	&	&\ddots	&\vdots	\\
	&	&	&#3#1_{#2#2}\\
\end{array}
}

\newcommand{\loww}[2]{\left(\begin{array} {cccc}
#1_{11}	&	&	&	\\
#1_{21}	&#1_{22}&	&	\\
\vdots	&\vdots	&\ddots	&	\\
#1_{#2 1}	&#1_{#2 2}&\cdots	&#1_{#2#2}\\
\end{array}
\right)}

\newcommand{\lowwm}[3]{\left(\begin{array} {cccc}
#3#1_{11}	&	&	&	\\
#1_{21}	&#3#1_{22}&	&	\\
\vdots	&\vdots	&\ddots	&	\\
#1_{#2 1}	&#1_{#2 2}&\cdots	&#3#1_{#2#2}\\
\end{array}
\right)}

\newcommand{\nlowwm}[3]{\begin{array} {cccc}
#3#1_{11}	&	&	&	\\
#1_{21}	&#3#1_{22}&	&	\\
\vdots	&\vdots	&\ddots	&	\\
#1_{#2 1}	&#1_{#2 2}&\cdots	&#3#1_{#2#2}\\
\end{array}
}

\newcommand{\mmss}[5]{\left(\begin{array} {cccccc}
#1_{11}	&#1_{12}&\cdots	&#1_{1#3}&\cdots& #1_{1#5}\\
#1_{21}	&#1_{22}&\cdots	&#1_{2#3}&\cdots& #1_{2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{{#2}1}&#1_{{#2}2}&\cdots&#1_{#2#3}&\cdots&#1_{#2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{#4 1}&#1_{#4 2}&\cdots&#1_{#4#3}&\cdots&#1_{#4#5}\\
\end{array}
\right)}

\newcommand{\diaaaa}[4]{\left(\begin{array} {cccc}
#1&&&\\
&#2&&\\
&&#3&\\
&&&#4\\
\end{array}
\right)}

\newcommand{\diag}[5]{\left(\begin{array} {cccccc}
#1&&&&&\\
&#2&&&&\\
&&#3&&&\\
&&&#4&&\\
&&&&\ddots&\\
&&&&&#5\\
\end{array}
\right)}

\newcommand{\ndiag}[5]{\begin{array} {cccccc}
#1&&&&&\\
&#2&&&&\\
&&#3&&&\\
&&&#4&&\\
&&&&\ddots&\\
&&&&&#5\\
\end{array}

}

\newcommand{\mmssr}[5]{\left(\begin{array} {cccccc}
#1_{11}	&#1_{12}&\cdots	&#1_{1#3}&\cdots& #1_{1#5}\\
#1_{21}	&#1_{22}&\cdots	&#1_{2#3}&\cdots& #1_{2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\\hline
\multicolumn{1}{|c}{#1_{{#2}1}}&#1_{{#2}2}&\cdots&#1_{#2#3}&\cdots&\multicolumn{1}{c|}{#1_{#2#5}}\\\hline
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{#4 1}&#1_{#4 2}&\cdots&#1_{#4#3}&\cdots&#1_{#4#5}\\
\end{array}
\right)}
\newcommand{\mmssc}[5]{\left(\begin{array} {ccc|c|cc}\cline{4-4}
#1_{11}	&#1_{12}&\cdots	&#1_{1#3}&\cdots& #1_{1#5}\\
#1_{21}	&#1_{22}&\cdots	&#1_{2#3}&\cdots& #1_{2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{{#2}1}&#1_{{#2}2}&\cdots&#1_{#2#3}&\cdots&#1_{#2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{#4 1}&#1_{#4 2}&\cdots&#1_{#4#3}&\cdots&#1_{#4#5}\\\cline{4-4}
\end{array}
\right)}

\newcommand{\mmssa}[5]{\left(\begin{array} {cccccc}
#1_{11}	&#1_{12}&\cdots	&#1_{1#3}&\cdots& #1_{1#5}\\
#1_{21}	&#1_{22}&\cdots	&#1_{2#3}&\cdots& #1_{2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\\cline{4-4}
#1_{{#2}1}&#1_{{#2}2}&\cdots&\multicolumn{1}{|c|}{#1_{#2#3}}&\cdots&#1_{#2#5}\\\cline{4-4}
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{#4 1}&#1_{#4 2}&\cdots&#1_{#4#3}&\cdots&#1_{#4#5}\\
\end{array}
\right)}


\newcommand{\mmps}[5]{\left(\begin{array} {cccc}
#1_{11}#5#2_{11}	&#1_{12}#5#2_{12}&\cdots	& #1_{1#4}#5#2_{1#4}\\
#1_{21}#5#2_{11}	&#1_{22}#5#2_{12}&\cdots	& #1_{2#4}#5#2_{2#4}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#1_{#3 1}#5#2_{#3 1}	&#1_{#3 2}#5#2_{#3 2}&\cdots	&#1_{#3#4}#5#2_{#3#4}\\
\end{array}
\right)}

\newcommand{\mmtps}[5]{\left(\begin{array} {cccc}
#1_{1}#5#2_{1}	&#1_{1}#5#2_{2}&\cdots	& #1_{1}#5#2_{#4}\\
#1_{2}#5#2_{1}	&#1_{2}#5#2_{2}&\cdots	& #1_{2}#5#2_{#4}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#1_{#3}#5#2_{1}	&#1_{#3}#5#2_{2}&\cdots	&#1_{#3}#5#2_{#4}\\
\end{array}
\right)}
\newcommand{\mmvts}[4]{\left(\begin{array} {cccc}
#1_{1}#2_{1}	&#1_{1}#2_{2}&\cdots	& #1_{1}#2_{#4}\\
#1_{2}#2_{1}	&#1_{2}#2_{2}&\cdots	& #1_{2}#2_{#4}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#1_{#3}#2_{1}	&#1_{#3}#2_{2}&\cdots	&#1_{#3}#2_{#4}\\
\end{array}
\right)}

\newcommand{\mmts}[4]{\left(\begin{array} {cccc}
\sum_{j=1}^n #1_{1j}#2_{j1}	&\sum_{j=1}^n #1_{1j}#2_{j2}&\cdots	& \sum_{j=1}^n #1_{1j}#2_{j#4}\\
\sum_{j=1}^n #1_{2j}#2_{j1}	&\sum_{j=1}^n #1_{2j}#2_{j2}&\cdots	& \sum_{j=1}^n #1_{2j}#2_{j#4}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
\sum_{j=1}^n #1_{#3j}#2_{j1}	&\sum_{j=1}^n #1_{#3j}#2_{j2}&\cdots	&\sum_{j=1}^n #1_{#3j}#2_{j#4}\\
\end{array}
\right)}


\newcommand{\rr}[2]{\begin{pmatrix}
#1 & #2\\
\end{pmatrix}}

\newcommand{\hrr}[2]{\left(\begin{array} {c;{2pt/2pt}c}
#1 & #2\\
\end{array}
\right)}

\newcommand{\nrr}[2]{\begin{array} {cc}
#1 & #2\\
\end{array}
}

\newcommand{\rrr}[3]{\left(\begin{array} {ccc}
#1 & #2 & #3\\
\end{array}
\right)}

\newcommand{\hrrr}[3]{\left(\begin{array} {c;{2pt/2pt}c;{2pt/2pt}c}
#1 & #2 & #3\\
\end{array}
\right)}

\newcommand{\nrrr}[3]{\begin{array} {ccc}
#1 & #2 & #3\\
\end{array}
}

\newcommand{\rrrr}[4]{\left(\begin{array} {cccc}
#1 & #2 & #3 & #4\\
\end{array}
\right)}

\newcommand{\hrrrr}[4]{\left(\begin{array} {c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c}
#1 & #2 & #3 & #4\\
\end{array}
\right)}

\newcommand{\nrrrr}[4]{\begin{array} {ccccc}
#1 & #2 & #3 & #4\\
\end{array}
}

\newcommand{\rrrrr}[5]{\left(\begin{array} {ccccc}
#1 & #2 & #3 & #4 & #5\\
\end{array}
\right)}

\newcommand{\hrrrrr}[5]{\left(\begin{array} {c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c}
#1 & #2 & #3 & #4 & #5\\
\end{array}
\right)}

\newcommand{\nrrrrr}[5]{\begin{array} {ccccc}
#1 & #2 & #3 & #4 & #5\\
\end{array}
}

\newcommand{\rrrrrr}[6]{\left(\begin{array} {cccccc}
#1 & #2 & #3 & #4 & #5 & #6\\
\end{array}
\right)}

\newcommand{\hrrrrrr}[6]{\left(\begin{array} {c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c}
#1 & #2 & #3 & #4 & #5 & #6\\
\end{array}
\right)}

\newcommand{\nhrrrrrr}[6]{\begin{array} {c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c}
#1 & #2 & #3 & #4 & #5 & #6\\
\end{array}
}

\newcommand{\nrrrrrr}[6]{\begin{array} {cccccc}
#1 & #2 & #3 & #4 & #5 & #6\\
\end{array}
}

\newcommand{\rrrrrrr}[7]{\left(\begin{array} {ccccccc}
#1 & #2 & #3 & #4 & #5 & #6 & #7\\
\end{array}
\right)}

\newcommand{\hrrrrrrr}[7]{\left(\begin{array} {c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c;}
#1 & #2 & #3 & #4 & #5 & #6& #7\\
\end{array}
\right)}

\newcommand{\nhrrrrrrr}[7]{\begin{array} {c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c;{2pt/2pt}c;}
#1 & #2 & #3 & #4 & #5 & #6 & #7\\
\end{array}
}

\newcommand{\nrrrrrrr}[7]{\begin{array} {ccccccc}
#1 & #2 & #3 & #4 & #5 & #6 & #7\\
\end{array}
}
\newcommand{\rrrrrrrr}[8]{\left(\begin{array} {cccccccc}
#1 & #2 & #3 & #4 & #5 & #6 & #7 & #8\\
\end{array}
\right)}
\newcommand{\rrrrrrrrr}[9]{\left(\begin{array} {ccccccccc}
#1 & #2 & #3 & #4 & #5 & #6 & #7 & #8 & #9\\
\end{array}
\right)}


\newcommand{\rrs}[2]{\left(\begin{array} {cccc}
#1{1}	&#1{2}&\cdots	&#1{#2}\\
\end{array}
\right)}

% Column Vectors
\newcommand{\cc}[2]{\begin{pmatrix}
#1\\
#2\\
\end{pmatrix}}

\newcommand{\ncc}[2]{\begin{array} {c}
#1\\
#2\\
\end{array}
}


\newcommand{\hcc}[2]{\left(\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\
\end{array}
\right)}

\newcommand{\ccc}[3]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
\end{array}
\right)}

\newcommand{\nccc}[3]{\begin{array} {c}
#1\\
#2\\
#3\\
\end{array}
}

\newcommand{\hccc}[3]{\left(\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\
\end{array}
\right)}


\newcommand{\cccc}[4]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
\end{array}
\right)}

\newcommand{\ncccc}[4]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
\end{array}
}

\newcommand{\hcccc}[4]{\left(\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\ \hdashline[2pt/2pt]
#4\\
\end{array}
\right)}
\newcommand{\ccccc}[5]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
\end{array}
\right)}

\newcommand{\nccccc}[5]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
\end{array}
}

\newcommand{\hccccc}[5]{\left(\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\ \hdashline[2pt/2pt]
#4\\ \hdashline[2pt/2pt]
#5\\
\end{array}
\right)}

\newcommand{\nhccccc}[5]{\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\ \hdashline[2pt/2pt]
#4\\ \hdashline[2pt/2pt]
#5\\
\end{array}
}

\newcommand{\cccccc}[6]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
\end{array}
\right)}

\newcommand{\ncccccc}[6]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
\end{array}
}

\newcommand{\hcccccc}[6]{\left(\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\ \hdashline[2pt/2pt]
#4\\ \hdashline[2pt/2pt]
#5\\ \hdashline[2pt/2pt]
#6\\
\end{array}
\right)}

\newcommand{\nhcccccc}[6]{\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\ \hdashline[2pt/2pt]
#4\\ \hdashline[2pt/2pt]
#5\\ \hdashline[2pt/2pt]
#6\\
\end{array}
}


\newcommand{\ccccccc}[7]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
\end{array}
\right)}

\newcommand{\nccccccc}[7]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
\end{array}
}

\newcommand{\hccccccc}[7]{\left(\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\ \hdashline[2pt/2pt]
#4\\ \hdashline[2pt/2pt]
#5\\ \hdashline[2pt/2pt]
#6\\ \hdashline[2pt/2pt]
#7\\
\end{array}
\right)}

\newcommand{\nhccccccc}[7]{\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\ \hdashline[2pt/2pt]
#4\\ \hdashline[2pt/2pt]
#5\\ \hdashline[2pt/2pt]
#6\\ \hdashline[2pt/2pt]
#7\\
\end{array}
}

\newcommand{\cccccccc}[8]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
#8\\
\end{array}
\right)}

\newcommand{\ncccccccc}[8]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
#8\\
\end{array}
}

\newcommand{\hcccccccc}[8]{\left(\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\ \hdashline[2pt/2pt]
#4\\ \hdashline[2pt/2pt]
#5\\ \hdashline[2pt/2pt]
#6\\ \hdashline[2pt/2pt]
#7\\ \hdashline[2pt/2pt]
#8\\
\end{array}
\right)}

\newcommand{\nhcccccccc}[8]{\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\ \hdashline[2pt/2pt]
#4\\ \hdashline[2pt/2pt]
#5\\ \hdashline[2pt/2pt]
#6\\ \hdashline[2pt/2pt]
#7\\ \hdashline[2pt/2pt]
#8\\
\end{array}
}


\newcommand{\ccccccccc}[9]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
#8\\
#9\\
\end{array}
\right)}

\newcommand{\nccccccccc}[9]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
#8\\
#9\\
\end{array}
}

\newcommand{\hccccccccc}[9]{\left(\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\ \hdashline[2pt/2pt]
#4\\ \hdashline[2pt/2pt]
#5\\ \hdashline[2pt/2pt]
#6\\ \hdashline[2pt/2pt]
#7\\ \hdashline[2pt/2pt]
#8\\ \hdashline[2pt/2pt]
#9\\
\end{array}
\right)}

\newcommand{\nhccccccccc}[9]{\begin{array} {c}
#1\\ \hdashline[2pt/2pt]
#2\\ \hdashline[2pt/2pt]
#3\\ \hdashline[2pt/2pt]
#4\\ \hdashline[2pt/2pt]
#5\\ \hdashline[2pt/2pt]
#6\\ \hdashline[2pt/2pt]
#7\\ \hdashline[2pt/2pt]
#8\\ \hdashline[2pt/2pt]
#9\\
\end{array}
}

\newcommand{\ccs}[3]{\left(\begin{array} {c}
#1_{1{#3}}\\
#1_{2{#3}}\\
\vdots\\
#1_{#2#3}\\
\end{array}
\right)}


==> PlainPaper/Command/linear.tex <==
%ini/Command
\makeatletter
\def\t{\@tt|\em\@gobble\@ttt}
\def\em\@tt#1\em{\@tt|\em}
\def\cm\@tt#1\em#2\@ttt{
\begin{tabular}{#1}
\hline
#2
\\\hline
\end{tabular}\@gobble
}
\def\@tt#1\@ttt#2{
\@ifnextchar,{\@tt #1 & #2\\\hline\expandafter\expandafter\expandafter\@gobble\expandafter\@gobble\@gobble\@ttt}{
\@ifnextchar.{\cm\@tt|l #1 & #2\@ttt}{\@tt|l #1 & #2\@ttt}
}
}

\def\m{\@tut\@gobble\@tutt}
\def\@tut#1\@tutt#2{
\@ifnextchar,{\@tut #1 & #2\\\expandafter\expandafter\expandafter\@gobble\expandafter\@gobble\@gobble\@tutt}{
\@ifnextchar.{\begin{pmatrix}#1 &#2\end{pmatrix}\@gobble}{\@tut #1 & #2\@tutt}
}
}

\def\bm{\@tuut\@gobble\@tuutt}
\def\@tuut#1\@tuutt#2{
\@ifnextchar,{\@tuut #1 & #2\cr\expandafter\expandafter\expandafter\@gobble\expandafter\@gobble\@gobble\@tuutt}{
\@ifnextchar.{\bordermatrix{#1 &#2\cr}\@gobble}{\@tuut #1 & #2\@tuutt}
}
}





\makeatother
\newcommand{\basis}[2]{\{#1_1,#1_2,\cdots,#1_#2\}}
\newcommand{\baba}[1]{\{#1_1,#1_2\}}
\newcommand{\bababa}[1]{\{#1_1,#1_2,#1_3\}}
\newcommand{\babababa}[1]{\{#1_1,#1_2,#1_3,#1_4\}}
\newcommand{\obaba}[1]{\m{#1_1}{#1_2}.}
\newcommand{\obababa}[1]{\m{#1_1}{#1_2}{#1_3}.}
\newcommand{\obabababa}[1]{\m{#1_1}{#1_2}{#1_3}{#1_4}.}
\newcommand{\tr}{\mathrm{tr}}

\newcommand{\obasis}[2]{\m {#1_1}{#1_2}{\cdots}{#1_#2}.}
\newcommand{\obasi}[2]{\m {#1_1}{\cdots}{#1_#2}.}
\newcommand{\truebasis}[2]{\rrrr{#1_1}{#1_2}{\cdots}{#1_#2}}
\newcommand{\coro}[2]{\m {#1_1},{#1_2},{\vdots},{#1_#2}.}
\newcommand{\coo}[2]{\m {#1_1},{\vdots},{#1_#2}.}
\newcommand{\coco}[1]{\m {#1_1},{#1_2}.}
\newcommand{\cococo}[1]{\m {#1_1},{#1_2},{#1_3}.}
\newcommand{\cocococo}[1]{\m {#1_1},{#1_2},{#1_3},{#1_4}.}
\newcommand{\coros}[4]{\cccc{#1_1#2#3_1}{#1_2#2#3_2}{\vdots}{#1_#4#2#3_#4}}
\newcommand{\corov}[3]{\cccc{#1_1#2}{#1_2#2}{\vdots}{#1_#3#2}}
%The following are only for examples
\newcommand{\rrce}[6]{\left(\begin{array} {ccc}\hline
\multicolumn{1}{|c}{#1} & #2	&\multicolumn{1}{c|}{#3}	\\\hline
#4 & #5	&#6	\\
\end{array}
\right)}

\newcommand{\ccre}[6]{\left(\begin{array} {c|c|}\cline{2-2}
#1 & #2	\\
#3 & #4	\\
#5 & #6	\\\cline{2-2}
\end{array}
\right)}

\newcommand{\mme}[4]{\left(\begin{array} {cc}\cline{2-2}
#1 & \multicolumn{1}{|c|}{#2}\\\cline{2-2}
#3 & #4\\
\end{array}
\right)}
%The following are for determinants

\newcommand{\dets}[4]{\left|\begin{array} {ccccc}
#1_{11}	&#1_{12}&#1_{13}&\cdots	& #1_{1#4}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#2 1}	&#1_{#2 2}&#1_{#2 3}&\cdots	& #1_{#2 #4}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#3 1}	&#1_{#3 2}&#1_{#3 3}&\cdots	& #1_{#3 #4}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#4 1}	&#1_{#4 2}&#1_{#4 3}&\cdots	& #1_{#4 #4}\\
\end{array}
\right|}

\newcommand{\detu}[3]{\left|\begin{array} {ccccc}
#1_{11}	&#1_{12}&#1_{13}&\cdots	& #1_{1#3}\\
        &#1_{2 2}&#1_{2 3}&\cdots	& #1_{2 #3}\\
        &       &#1_{#2 3}&\cdots	& #1_{#2 #3}\\
    	&      &    	&\cdots	&\cdots	\\
	&&&   & #1_{#3 #3}\\
\end{array}
\right|}

\newcommand{\detdia}[4]{\left|\begin{array} {ccccc}
#1	&    &      &       &       \\
        &#2&      &   	&       \\
        &       &#3& 	&       \\
    	&      &    	&\ddots	&	\\
	&&&   & #4\\
\end{array}
\right|}

\newcommand{\deta}[5]{\left|\begin{array} {ccccc}
#1_{11}	&#1_{12}&#1_{13}&\cdots	& #1_{1#5}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#3 1}+#2 #1_{#4 1}	&#1_{#3 2}+#2 #1_{#4 2}&#1_{#3 3}+#2 #1_{#4 3}&\cdots	& #1_{#3 #5}+#2 #1_{#4 #5}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#4 1}	&#1_{#4 2}&#1_{#4 3}&\cdots	& #1_{#4 #5}\\
\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#5 1}	&#1_{#5 2}&#1_{#5 3}&\cdots	& #1_{#5 #5}\\
\end{array}
\right|}

%\newcommand{\detaa}[5]{\left|\begin{array} {ccccc}
%#1_{11}	&#1_{12}&#1_{13}&\cdots	& #1_{1#5}\\
%\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
%#1_{#3 1}+#2_{#4 1}	&#1_{#3 2}+#2_{#4 2}&#1_{#3 3}+#2_{#4 3}&\cdots	& #1_{#3 %#5}+#2_{#4 #5}\\
%\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
%#1_{#4 1}	&#1_{#4 2}&#1_{#4 3}&\cdots	& #1_{#4 #5}\\
%\cdots	&\cdots	&\cdots	&\cdots	&\cdots	\\
%#1_{#5 1}	&#1_{#5 2}&#1_{#5 3}&\cdots	& #1_{#5 #5}\\
%\end{array}
%\right|}

\newcommand{\dett}[1]{\left|\begin{array}{c}#1\end{array}\right|}

\newcommand{\detaao}[4]{\left|\begin{array} {cccc}
#1_{11}	&#1_{12}&\cdots	& #1_{1#4}\\
\cdots	&\cdots	&\cdots	&\cdots\\
#2_{#3 1}	&#2_{#3 1}&\cdots	& #2_{#3 1}\\
\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#4 1}	&#1_{#4 2}&\cdots	& #1_{#4 #4}\\
\end{array}
\right|}

\newcommand{\detaa}[4]{\left|\begin{array} {cccc}
#1_{11}	&#1_{12}&\cdots	& #1_{1#4}\\
\cdots	&\cdots	&\cdots	&\cdots\\
#2_{#3 1}+#1_{#3 1}	&#2_{#3 1}+#1_{#3 2}&\cdots	& #2_{#3 1}+#1_{#3 #4}\\
\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#4 1}	&#1_{#4 2}&\cdots	& #1_{#4 #4}\\
\end{array}
\right|}

\newcommand{\detm}[4]{\left|\begin{array} {cccc}
#1_{11}	&#1_{12}&\cdots	& #1_{1#4}\\
\cdots	&\cdots	&\cdots	&\cdots\\
#2#1_{#3 1}	&#2#1_{#3 2}&\cdots	& #2#1_{#3 #4}\\
\cdots	&\cdots	&\cdots	&\cdots	\\
#1_{#4 1}	&#1_{#4 2}&\cdots	& #1_{#4 #4}\\
\end{array}
\right|}
%The following are for elementary matrices

\newcommand{\elm}[2]{\bordermatrix{%
& 	&	&i	&	&	\cr
&#1 	&	&	&	&	\cr
&	&\ddots	&	&	&	\cr
i&	&	&#2	&	&	\cr
&	&	&	&\ddots	&	\cr
&	&	&	&	&#1	\cr
}}
\newcommand{\els}[1]{\bordermatrix{
& 	&	&	&	&	&	&	\cr
&#1 	&	&	&	&	&	&	\cr
&	&\ddots	&	&	&	&	&	\cr
i&	&	&0	&	&#1	&	&	\cr
&	&	&	&\ddots	&	&	&	\cr
j&	&	&#1	&	&0	&	&	\cr
&	&	&	&	&	&\ddots	&	\cr
&	&	&	&	&	&	&#1	\cr
}}

\newcommand{\ela}[2]{\bordermatrix{
& 	&	&	&	&j	&	&	\cr
&#1 	&	&	&	&	&	&	\cr
&	&\ddots	&	&	&	&	&	\cr
i&	&	&#1	&	&#2	&	&	\cr
&	&	&	&\ddots	&	&	&	\cr
&	&	&	&	&#1	&	&	\cr
&	&	&	&	&	&\ddots	&	\cr
&	&	&	&	&	&	&#1	\cr
}}

%The following are some some particular Matrices.
\newcommand{\mat}[5]{(#1_{#2#3})_{\substack{1\leq #2 \leq #4 \\ 1\leq #3 \leq #5}}}
\newcommand{\mato}[5]{(#1)_{\substack{1\leq #2 \leq #4 \\ 1\leq #3 \leq #5}}}

\newcommand{\mm}[4]{\left(\begin{array} {cc}
#1 & #2\\
#3 & #4\\
\end{array}
\right)}

\newcommand{\nmm}[4]{\begin{array} {cc}
#1 & #2\\
#3 & #4\\
\end{array}
}

\newcommand{\hmm}[4]{\left(\begin{array} {c|c}
#1 & #2\\ \hline
#3 & #4\\
\end{array}
\right)}

\newcommand{\nhmm}[4]{\begin{array} {c|c}
#1 & #2\\ \hline
#3 & #4\\
\end{array}
}

\newcommand{\rrc}[6]{\left(\begin{array} {ccc}
#1 & #2	&#3	\\
#4 & #5	&#6	\\
\end{array}
\right)}

\newcommand{\nrrc}[6]{\begin{array} {ccc}
#1 & #2	&#3	\\
#4 & #5	&#6	\\
\end{array}
}


\newcommand{\ccr}[6]{\left(\begin{array} {cc}
#1 & #2	\\
#3 & #4	\\
#5 & #6	\\
\end{array}
\right)}

\newcommand{\nccr}[6]{\begin{array} {cc}
#1 & #2	\\
#3 & #4	\\
#5 & #6	\\
\end{array}
}


\newcommand{\mmm}[9]{\left(\begin{array} {ccc}
#1 & #2 & #3\\
#4 & #5 & #6\\
#7 & #8 & #9\\
\end{array}
\right)}

\newcommand{\hmmm}[9]{\left(\begin{array} {c|c|c}
#1 & #2 & #3\\ \hline
#4 & #5 & #6\\ \hline
#7 & #8 & #9\\
\end{array}
\right)}

\newcommand{\nmmm}[9]{\begin{array} {ccc}
#1 & #2 & #3\\
#4 & #5 & #6\\
#7 & #8 & #9\\
\end{array}
}

\newcommand{\mms}[3]{\left(\begin{array} {cccc}
#1_{11}	&#1_{12}&\cdots	& #1_{1#3}\\
#1_{21}	&#1_{22}&\cdots	& #1_{2#3}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#1_{#2 1}	&#1_{#2 2}&\cdots	&#1_{#2#3}\\
\end{array}
\right)}


\newcommand{\mmhrs}[3]{\hrrrr{\ncccc{#1_{11}}{#1_{21}}{\vdots}{#1_{#2 1}}}{\ncccc{#1_{12}}{#1_{22}}{\vdots}{#1_{#1 2}}}{\ncccc{\cdots}{\cdots}{\ddots}{\cdots}}{\ncccc{#1_{1#3}}{b_{2#3}}{\vdots}{b_{#2#3}}}}

\newcommand{\mmhcs}[3]{\hcccc{\nrrrr{#1_{11}}{#1_{12}}{\cdots}{#1_{1#2 }}}{\nrrrr{#1_{21}}{#1_{22}}{\cdots}{#1_{2#1}}}{\nrrrr{\vdots}{\vdots}{\ddots}{\vdots}}{\nrrrr{#1_{#3 1}}{b_{#3 #2}}{\cdots}{b_{#2#3}}}}


\newcommand{\mmtrs}[3]{\left(\begin{array} {cccc}
#1_{11}	&#1_{21}&\cdots	& #1_{#3 1}\\
#1_{12}	&#1_{22}&\cdots	& #1_{#3 2}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#1_{1#2}	&#1_{2#2}&\cdots	&#1_{#3#2}\\
\end{array}
\right)}

\newcommand{\mmmm}[3]{\left(\begin{array} {cccc}
#111	&#121 &\cdots	& #1#31\\
#112	&#122 &\cdots	& #1#32\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#11#2	&#12#2&\cdots	&#1#3#2\\
\end{array}
\right)}

\newcommand{\upper}[2]{\left(\begin{array} {cccc}
#1_{11}	&#1_{12}&\cdots	& #1_{1#2}\\
	&#1_{22}&\cdots	& #1_{2#2}\\
	&	&\ddots	&\vdots	\\
	&	&	&#1_{#2#2}\\
\end{array}
\right)}

\newcommand{\upperm}[3]{\left(\begin{array} {cccc}
#3#1_{11}	&#1_{12}&\cdots	& #1_{1#2}\\
	&#3#1_{22}&\cdots	& #1_{2#2}\\
	&	&\ddots	&\vdots	\\
	&	&	&#3#1_{#2#2}\\
\end{array}
\right)}

\newcommand{\nupperm}[3]{\begin{array} {cccc}
#3#1_{11}	&#1_{12}&\cdots	& #1_{1#2}\\
	&#3#1_{22}&\cdots	& #1_{2#2}\\
	&	&\ddots	&\vdots	\\
	&	&	&#3#1_{#2#2}\\
\end{array}
}

\newcommand{\loww}[2]{\left(\begin{array} {cccc}
#1_{11}	&	&	&	\\
#1_{21}	&#1_{22}&	&	\\
\vdots	&\vdots	&\ddots	&	\\
#1_{#2 1}	&#1_{#2 2}&\cdots	&#1_{#2#2}\\
\end{array}
\right)}

\newcommand{\lowwm}[3]{\left(\begin{array} {cccc}
#3#1_{11}	&	&	&	\\
#1_{21}	&#3#1_{22}&	&	\\
\vdots	&\vdots	&\ddots	&	\\
#1_{#2 1}	&#1_{#2 2}&\cdots	&#3#1_{#2#2}\\
\end{array}
\right)}

\newcommand{\nlowwm}[3]{\begin{array} {cccc}
#3#1_{11}	&	&	&	\\
#1_{21}	&#3#1_{22}&	&	\\
\vdots	&\vdots	&\ddots	&	\\
#1_{#2 1}	&#1_{#2 2}&\cdots	&#3#1_{#2#2}\\
\end{array}
}

\newcommand{\mmss}[5]{\left(\begin{array} {cccccc}
#1_{11}	&#1_{12}&\cdots	&#1_{1#3}&\cdots& #1_{1#5}\\
#1_{21}	&#1_{22}&\cdots	&#1_{2#3}&\cdots& #1_{2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{{#2}1}&#1_{{#2}2}&\cdots&#1_{#2#3}&\cdots&#1_{#2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{#4 1}&#1_{#4 2}&\cdots&#1_{#4#3}&\cdots&#1_{#4#5}\\
\end{array}
\right)}

\newcommand{\diaaaa}[4]{\left(\begin{array} {cccc}
#1&&&\\
&#2&&\\
&&#3&\\
&&&#4\\
\end{array}
\right)}

\newcommand{\diag}[5]{\left(\begin{array} {cccccc}
#1&&&&&\\
&#2&&&&\\
&&#3&&&\\
&&&#4&&\\
&&&&\ddots&\\
&&&&&#5\\
\end{array}
\right)}

\newcommand{\ndiag}[5]{\begin{array} {cccccc}
#1&&&&&\\
&#2&&&&\\
&&#3&&&\\
&&&#4&&\\
&&&&\ddots&\\
&&&&&#5\\
\end{array}

}

\newcommand{\mmssr}[5]{\left(\begin{array} {cccccc}
#1_{11}	&#1_{12}&\cdots	&#1_{1#3}&\cdots& #1_{1#5}\\
#1_{21}	&#1_{22}&\cdots	&#1_{2#3}&\cdots& #1_{2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\\hline
\multicolumn{1}{|c}{#1_{{#2}1}}&#1_{{#2}2}&\cdots&#1_{#2#3}&\cdots&\multicolumn{1}{c|}{#1_{#2#5}}\\\hline
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{#4 1}&#1_{#4 2}&\cdots&#1_{#4#3}&\cdots&#1_{#4#5}\\
\end{array}
\right)}
\newcommand{\mmssc}[5]{\left(\begin{array} {ccc|c|cc}\cline{4-4}
#1_{11}	&#1_{12}&\cdots	&#1_{1#3}&\cdots& #1_{1#5}\\
#1_{21}	&#1_{22}&\cdots	&#1_{2#3}&\cdots& #1_{2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{{#2}1}&#1_{{#2}2}&\cdots&#1_{#2#3}&\cdots&#1_{#2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{#4 1}&#1_{#4 2}&\cdots&#1_{#4#3}&\cdots&#1_{#4#5}\\\cline{4-4}
\end{array}
\right)}

\newcommand{\mmssa}[5]{\left(\begin{array} {cccccc}
#1_{11}	&#1_{12}&\cdots	&#1_{1#3}&\cdots& #1_{1#5}\\
#1_{21}	&#1_{22}&\cdots	&#1_{2#3}&\cdots& #1_{2#5}\\
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\\cline{4-4}
#1_{{#2}1}&#1_{{#2}2}&\cdots&\multicolumn{1}{|c|}{#1_{#2#3}}&\cdots&#1_{#2#5}\\\cline{4-4}
\vdots	&\vdots	&\ddots	&\vdots	&\ddots	&\vdots	\\
#1_{#4 1}&#1_{#4 2}&\cdots&#1_{#4#3}&\cdots&#1_{#4#5}\\
\end{array}
\right)}


\newcommand{\mmps}[5]{\left(\begin{array} {cccc}
#1_{11}#5#2_{11}	&#1_{12}#5#2_{12}&\cdots	& #1_{1#4}#5#2_{1#4}\\
#1_{21}#5#2_{11}	&#1_{22}#5#2_{12}&\cdots	& #1_{2#4}#5#2_{2#4}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#1_{#3 1}#5#2_{#3 1}	&#1_{#3 2}#5#2_{#3 2}&\cdots	&#1_{#3#4}#5#2_{#3#4}\\
\end{array}
\right)}

\newcommand{\mmtps}[5]{\left(\begin{array} {cccc}
#1_{1}#5#2_{1}	&#1_{1}#5#2_{2}&\cdots	& #1_{1}#5#2_{#4}\\
#1_{2}#5#2_{1}	&#1_{2}#5#2_{2}&\cdots	& #1_{2}#5#2_{#4}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#1_{#3}#5#2_{1}	&#1_{#3}#5#2_{2}&\cdots	&#1_{#3}#5#2_{#4}\\
\end{array}
\right)}
\newcommand{\mmvts}[4]{\left(\begin{array} {cccc}
#1_{1}#2_{1}	&#1_{1}#2_{2}&\cdots	& #1_{1}#2_{#4}\\
#1_{2}#2_{1}	&#1_{2}#2_{2}&\cdots	& #1_{2}#2_{#4}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
#1_{#3}#2_{1}	&#1_{#3}#2_{2}&\cdots	&#1_{#3}#2_{#4}\\
\end{array}
\right)}

\newcommand{\mmts}[4]{\left(\begin{array} {cccc}
\sum_{j=1}^n #1_{1j}#2_{j1}	&\sum_{j=1}^n #1_{1j}#2_{j2}&\cdots	& \sum_{j=1}^n #1_{1j}#2_{j#4}\\
\sum_{j=1}^n #1_{2j}#2_{j1}	&\sum_{j=1}^n #1_{2j}#2_{j2}&\cdots	& \sum_{j=1}^n #1_{2j}#2_{j#4}\\
\vdots	&\vdots	&\ddots	&\vdots	\\
\sum_{j=1}^n #1_{#3j}#2_{j1}	&\sum_{j=1}^n #1_{#3j}#2_{j2}&\cdots	&\sum_{j=1}^n #1_{#3j}#2_{j#4}\\
\end{array}
\right)}


\newcommand{\rr}[2]{\left(\begin{array} {cc}
#1 & #2\\
\end{array}
\right)}

\newcommand{\hrr}[2]{\left(\begin{array} {c|c}
#1 & #2\\
\end{array}
\right)}

\newcommand{\nrr}[2]{\begin{array} {cc}
#1 & #2\\
\end{array}
}

\newcommand{\rrr}[3]{\left(\begin{array} {ccc}
#1 & #2 & #3\\
\end{array}
\right)}

\newcommand{\hrrr}[3]{\left(\begin{array} {c|c|c}
#1 & #2 & #3\\
\end{array}
\right)}

\newcommand{\nrrr}[3]{\begin{array} {ccc}
#1 & #2 & #3\\
\end{array}
}

\newcommand{\rrrr}[4]{\left(\begin{array} {cccc}
#1 & #2 & #3 & #4\\
\end{array}
\right)}

\newcommand{\hrrrr}[4]{\left(\begin{array} {c|c|c|c}
#1 & #2 & #3 & #4\\
\end{array}
\right)}

\newcommand{\nrrrr}[4]{\begin{array} {ccccc}
#1 & #2 & #3 & #4\\
\end{array}
}

\newcommand{\rrrrr}[5]{\left(\begin{array} {ccccc}
#1 & #2 & #3 & #4 & #5\\
\end{array}
\right)}

\newcommand{\hrrrrr}[5]{\left(\begin{array} {c|c|c|c|c}
#1 & #2 & #3 & #4 & #5\\
\end{array}
\right)}

\newcommand{\nrrrrr}[5]{\begin{array} {ccccc}
#1 & #2 & #3 & #4 & #5\\
\end{array}
}

\newcommand{\rrrrrr}[6]{\left(\begin{array} {cccccc}
#1 & #2 & #3 & #4 & #5 & #6\\
\end{array}
\right)}

\newcommand{\hrrrrrr}[6]{\left(\begin{array} {c|c|c|c|c}
#1 & #2 & #3 & #4 & #5 & #6\\
\end{array}
\right)}

\newcommand{\nhrrrrrr}[6]{\begin{array} {c|c|c|c|c}
#1 & #2 & #3 & #4 & #5 & #6\\
\end{array}
}

\newcommand{\nrrrrrr}[6]{\begin{array} {cccccc}
#1 & #2 & #3 & #4 & #5 & #6\\
\end{array}
}

\newcommand{\rrrrrrr}[7]{\left(\begin{array} {ccccccc}
#1 & #2 & #3 & #4 & #5 & #6 & #7\\
\end{array}
\right)}

\newcommand{\hrrrrrrr}[7]{\left(\begin{array} {c|c|c|c|c|c|c;}
#1 & #2 & #3 & #4 & #5 & #6& #7\\
\end{array}
\right)}

\newcommand{\nhrrrrrrr}[7]{\begin{array} {c|c|c|c|c|c|c;}
#1 & #2 & #3 & #4 & #5 & #6 & #7\\
\end{array}
}

\newcommand{\nrrrrrrr}[7]{\begin{array} {ccccccc}
#1 & #2 & #3 & #4 & #5 & #6 & #7\\
\end{array}
}
\newcommand{\rrrrrrrr}[8]{\left(\begin{array} {cccccccc}
#1 & #2 & #3 & #4 & #5 & #6 & #7 & #8\\
\end{array}
\right)}
\newcommand{\rrrrrrrrr}[9]{\left(\begin{array} {ccccccccc}
#1 & #2 & #3 & #4 & #5 & #6 & #7 & #8 & #9\\
\end{array}
\right)}


\newcommand{\rrs}[2]{\left(\begin{array} {cccc}
#1{1}	&#1{2}&\cdots	&#1{#2}\\
\end{array}
\right)}

% Column Vectors
\newcommand{\cc}[2]{\begin{pmatrix}
#1\\
#2\\
\end{pmatrix}}

\newcommand{\ncc}[2]{\begin{array} {c}
#1\\
#2\\
\end{array}
}


\newcommand{\hcc}[2]{\left(\begin{array} {c}
#1\\ \hline
#2\\
\end{array}
\right)}

\newcommand{\ccc}[3]{\begin{pmatrix}
#1\\
#2\\
#3\\
\end{pmatrix}
}

\newcommand{\nccc}[3]{\begin{array} {c}
#1\\
#2\\
#3\\
\end{array}
}

\newcommand{\hccc}[3]{\left(\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\
\end{array}
\right)}


\newcommand{\cccc}[4]{\begin{pmatrix}
#1\\
#2\\
#3\\
#4\\
\end{pmatrix}}

\newcommand{\ncccc}[4]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
\end{array}
}

\newcommand{\hcccc}[4]{\left(\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\ \hline
#4\\
\end{array}
\right)}
\newcommand{\ccccc}[5]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
\end{array}
\right)}

\newcommand{\nccccc}[5]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
\end{array}
}

\newcommand{\hccccc}[5]{\left(\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\ \hline
#4\\ \hline
#5\\
\end{array}
\right)}

\newcommand{\nhccccc}[5]{\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\ \hline
#4\\ \hline
#5\\
\end{array}
}

\newcommand{\cccccc}[6]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
\end{array}
\right)}

\newcommand{\ncccccc}[6]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
\end{array}
}

\newcommand{\hcccccc}[6]{\left(\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\ \hline
#4\\ \hline
#5\\ \hline
#6\\
\end{array}
\right)}

\newcommand{\nhcccccc}[6]{\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\ \hline
#4\\ \hline
#5\\ \hline
#6\\
\end{array}
}


\newcommand{\ccccccc}[7]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
\end{array}
\right)}

\newcommand{\nccccccc}[7]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
\end{array}
}

\newcommand{\hccccccc}[7]{\left(\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\ \hline
#4\\ \hline
#5\\ \hline
#6\\ \hline
#7\\
\end{array}
\right)}

\newcommand{\nhccccccc}[7]{\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\ \hline
#4\\ \hline
#5\\ \hline
#6\\ \hline
#7\\
\end{array}
}

\newcommand{\cccccccc}[8]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
#8\\
\end{array}
\right)}

\newcommand{\ncccccccc}[8]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
#8\\
\end{array}
}

\newcommand{\hcccccccc}[8]{\left(\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\ \hline
#4\\ \hline
#5\\ \hline
#6\\ \hline
#7\\ \hline
#8\\
\end{array}
\right)}

\newcommand{\nhcccccccc}[8]{\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\ \hline
#4\\ \hline
#5\\ \hline
#6\\ \hline
#7\\ \hline
#8\\
\end{array}
}


\newcommand{\ccccccccc}[9]{\left(\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
#8\\
#9\\
\end{array}
\right)}

\newcommand{\nccccccccc}[9]{\begin{array} {c}
#1\\
#2\\
#3\\
#4\\
#5\\
#6\\
#7\\
#8\\
#9\\
\end{array}
}

\newcommand{\hccccccccc}[9]{\left(\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\ \hline
#4\\ \hline
#5\\ \hline
#6\\ \hline
#7\\ \hline
#8\\ \hline
#9\\
\end{array}
\right)}

\newcommand{\nhccccccccc}[9]{\begin{array} {c}
#1\\ \hline
#2\\ \hline
#3\\ \hline
#4\\ \hline
#5\\ \hline
#6\\ \hline
#7\\ \hline
#8\\ \hline
#9\\
\end{array}
}

\newcommand{\ccs}[3]{\left(\begin{array} {c}
#1_{1{#3}}\\
#1_{2{#3}}\\
\vdots\\
#1_{#2#3}\\
\end{array}
\right)}


==> PlainPaper/Command/polynomial.tex <==
\newcommand{\lPP}[4]{P_{2,#1}=\{#2#1^2+#3#1+#4,\text{ where }#2,#3,#4\in \CC\}}
\newcommand{\lP}[3]{P_{1,#1}=\{#2#1+#3,\text{ where }#2,#3\in \CC\}}
\newcommand{\lPPP}[5]{P_{3,#1}=\{#2#1^3+#3#1^2+#4#1+#5,\text{ where }#2,#3,#4,#5\in \CC\}}


==> PlainPaper/Command/tableau.tex <==
\newcommand{\nl}[2]{\dim\left(\ker(#1^{#2})\right)}
\newcommand{\td}{
{Tableau Direction} 

\[zzz]{\B{$\ww$}\B{$\vv$}}
:$\ww=T\vv$
}
\newcommand{\TD}{
{\bf \text{Tableau Direction }}
\ytableaushort{\ww\vv}:$\ww=T\vv$
}
\newcommand{\TDD}[1]{
{\bf \text{Tableau Direction }}

\ytableaushort{\ww\vv}:$\ww=#1\vv$
}

\newcommand{\yt}{\ytableaushort}
\newcommand{\yd}{\ydiagram}
\newcommand{\ys}{\ytableausetup{mathmode, boxsize=1em}}
\newcommand{\ym}{\ytableausetup{mathmode, boxsize=1.5em}}
\newcommand{\yl}{\ytableausetup{mathmode, boxsize=2.5em}}



==> PlainPaper/etc.tex <==
 


==> PlainPaper/inh.tex <==
Style:Style
Title:Title
Author:Author
FontSize:FontSize
Status:Status


==> PlainPaper/ini.tex <==
 


==> PlainPaper/script.tex <==
\Road{ini}
\Road{inh}
\Road{etc}
\Road{plain}
\useas{Style}\Fixload


==> ini.tex <==
Template:plainpaper
Style:plain
Paper:lifting
FontSize:12pt
Status:a


==> script.tex <==
\def\reserve#1#2{\def\coffee##1{#2{#1}{##1}}}
\useas{Paper}\reserve\LoadTemplate\useas{Template}\coffee

